OPAL a Versatile Tool for Charged Particle Accelerator Simulations

Many sophisticated computer models have been developed to understand the behaviour of particle accelerators. Even these complex models often do not describe the measured data. Interactions of the beam with external fields, other particles in the same beam and the beam walls all present modelling challenges. These can be challenging to model correctly even with modern supercomputers. This paper describes OPAL (Object Oriented Parallel Accelerator Library), a parallel open source tool for charged-particle optics in linear accelerators and rings, including 3D space charge. OPAL is built from the ground up as a parallel application exemplifying the fact that high performance computing is the third leg of science, complementing theory and experiment. Using the MAD language with extensions, OPAL can run on a laptop as well as on the largest high performance computing systems. The OPAL framework makes it easy to add new features in the form of new C++ classes, enabling the modelling of many physics processes and field types. OPAL comes in two flavours: OPAL-cycl: tracks particles with 3D space charge including neighbouring turns in cyclotrons and FFAs with time as the independent variable. OPAL-t: models beam lines, linacs, rf-photo injectors and complete XFELs excluding the undulator. The code is managed through the git distributed version control system. A suite of unit tests have been developed for various parts of OPAL, validating each part of the code independently. System tests validate the overall integration of different elements.

==> contrib/autophase.tex <==
% !TEX root = ../main.tex


==> contrib/berlinapp.tex <==
% !TEX root = ../main.tex


==> contrib/concl.tex <==
% !TEX root = ../main.tex
\subsection{Future plans (all)} \label{ssec:future}


==> contrib/mpactapp.tex <==
% !TEX root = ../main.tex
%
% only comparison with the Anza paper

%Describe simple model and benchmark the Anza model. Then cite  \cite{ciae-rf-2013}. The description can very well be
%the HB Morschach conference paper.
Dark current and multipacting phenomena have been observed in various RF
structures of accelerators, e.g. \cite{DE}\cite{CY}. These phenomena are usually
harmful to the equipment and beam quality, as they will cause galvanic
etching on the surface of the cavity and thus cause RF breakdown. We have extended \opal to be a feasible tool
for performing large scale dark current and multipacting simulations. This would
allow more thorough analysis and a deeper understanding of these phenomena.
Accurate simulations could lead to methods how these situations can be prevented
or diminished. 
To achieve these goals, first we introduce a particle-boundary collision test
model into \opal to facilitate the particle searching during tracking process. In
a subsequent step we add surface physics models including an analytic
Fowler-Nordheim field emission model and two secondary emission
models to \opal.

%The Child-Langmuir space charge model for emitted electrons is discussed here. A
%multigrid preconditioned iterative space charge solver able to treat
%complicated boundaries with higher accuracy is still work in progress and will
%be incorporated in the near future.

Complex 3D geometries are represented as triangulated surface
meshes. Subsequently we can make use of efficient 3D line segment-triangle
intersection (LSTI) tests to find particle-boundary collisions. Since we need to
precompute all triangle normals for triangle orientation anyway we can make use
of a fast algorithm relaying on having triangle normals available \cite{LT}.
In order to compute a LSTI we need the starting and end point of the
line segment under consideration, triangle vertices and normal. A schematic view
is sketched in Figure \ref{fig:L-T}.
%
\begin{figure}
\begin{center}
\input{figs/Line_Triangle.tikz}
\end{center}
\caption{Line segment-triangle intersection.\label{fig:L-T}}
\end{figure}
%
Vectors are denoted with arrows (i.e. $\vec{n}$), points (here in
$\mathcal{R}^3$) are bold (i.e. $\mathbf{x}_0$) and the remaining symbols denote
scalars. The algorithm for handling LSTI is given in Algorithm \ref{alg:lsti}.
%
\begin{algorithm}
  \caption{LSTI} \label{alg:lsti}
   \begin{algorithmic}[1]
     %\STATE \textbf{procedure} LSTI(\textbf{In:} line segment $\mathbf{x}_1-\mathbf{x}_0$, $\Delta(\mathbf{t}_0, \mathbf{t}_1, \mathbf{t}_2)$, \textbf{Out:} true $ \&\ \mathbf{I}$ or false)
     \STATE \textbf{procedure} LSTI(\textbf{In:} $\mathbf{x}_0$, $\mathbf{x}_1$, $\Delta(\mathbf{t}_0, \mathbf{t}_1, \mathbf{t}_2)$, \textbf{Out:} isInside, $\mathbf{I}$)
     \IF{$\vec{n} \cdot (\mathbf{x}_1-\mathbf{x}_0)=0$}
     \RETURN false \COMMENT{$\mathbf{x}_1-\mathbf{x}_0~||~\Delta \rightarrow$ no intersection}
     \ELSE
     \STATE $ r_i \leftarrow \frac{\vec{n} \cdot (\mathbf{t}_0-\mathbf{x}_0)}{ \vec{n}\cdot(\mathbf{x}_1-\mathbf{x}_0)} $
     \STATE $\mathbf{I} \leftarrow \mathbf{x}_0+r_i(\mathbf{x}_1-\mathbf{x}_0) $ \COMMENT {The intersection point of the line segment and planed}
     \IF{$ r_i $$<$$ 0$ \textbf{or} $ r_i$ $>$ $1 $}
        \RETURN false \COMMENT{early rejection: intersection is on the extension of line segment}
     \ELSE 
        \STATE \COMMENT{Check if the intersection point is inside the triangle}
        %\STATE The parametric plane equation: $ \mathbf{t}(s_i,t_i)=\mathbf{t}_0+s_i (\mathbf{t}_1-\mathbf{t}_0)+t_i(\mathbf{t}_2-\mathbf{t}_0)=\mathbf{t}_0+s_i\vec{u}+t_i\vec{v} $. As $\vec{w}=\mathbf{I}-\mathbf{t}_0$ is also in the plane, 
        \STATE Solve: $\vec{w}=\mathbf{t}_0+s_i\vec{u}+t_i\vec{v}$ \COMMENT{parametric plane equation}
        \STATE $s_i \leftarrow \frac{(\vec{u} \cdot \vec{v})(\vec{w} \cdot \vec{v})-(\vec{v} \cdot \vec{v})(\vec{w} \cdot \vec{u})}{(\vec{u} \cdot \vec{v})^2-(\vec{u} \cdot \vec{u})(\vec{v} \cdot \vec{v})}$
        \STATE $t_i \leftarrow \frac{(\vec{u} \cdot \vec{v})(\vec{w} \cdot \vec{u})-(\vec{u} \cdot \vec{u})(\vec{w} \cdot \vec{v})}{(\vec{u} \cdot \vec{v})^2-(\vec{u} \cdot \vec{u})(\vec{v} \cdot \vec{v})}$
        \IF{$ s_i \geq 0 $ \textbf{and} $ t_i \geq 0 $ \textbf{and} $ s_i+t_i \leq 1 $} 
            \RETURN (true, $\mathbf{I}$)
        \ELSE
            \RETURN false \COMMENT{no intersection between line segment and triangle}
        \ENDIF
     \ENDIF
\ENDIF
       \STATE \textbf{end procedure}
   \end{algorithmic}
 \end{algorithm}

Even though the implemented LSTI algorithm using precomputed triangle normal is
fast a huge number of LSTI calls are necessary. If we have $M$ triangles and $N$
particles in the simulation, both in the magnitude of hundreds of thousand to
millions, the number of LSTI tests in single time step without a early rejection
strategy would be $M \times N$, i.e., at least $10^{10}$ per time step.
Obviously, effective early rejection strategies (see Figure~\ref{fig:P-B}) are
needed to reduce the number of LSTI tests.


\begin{figure}[H]
    \begin{center}
        \input{figs/2d_grid.tikz}
    \end{center}
    \caption{Schematic view of particle-boundary early rejection strategy. The dark
    black line represents the boundary surface, particles are colored dots with an
    attached momenta arrow and inward normals gray arrows.\label{fig:P-B}}
\end{figure}

Assuming we need to determine whether a particle with position $\mathbf{r}$
and momenta $\mathbf{p}$ hits the boundary within time step $\Delta{t}$ we apply
the following early rejection strategies:
\begin{itemize}
    \item Test if the particle is near the boundary by checking if $\mathbf{r}$
    is inside the boundary bounding boxes (illustrated by gray grids in
    Figure ~\ref{fig:P-B}). 
    \item If $\mathbf{r}$ is not in a bounding box (green particle in Figure
    ~\ref{fig:P-B}), the particle is enough far away from boundary and
    can be integrated directly.
    \item If $\mathbf{r}$ is in a bounding box (yellow particle and red particle
    in Figure ~\ref{fig:P-B}), then we check all triangles in the bounding box
    (of the corresponding particle) as well as triangles in the adjacent 26
    bounding boxes to see if the momenta of the particle has a opposite
    direction with those triangles' normals.
    \item If the momenta and triangle normal are not opposite for all triangles
    checked (the yellow particle) do particle integration.
    \item If they are opposite (red particle) check if the particle has an
    intersection with the triangles by performing the LSTI test for each
    triangle. If an intersection exists the particle will hit the boundary
    during the current time step.
\end{itemize}

Field emission is a major source of both dark current particles and primary
incident particles in secondary emission. The Fowler-Nordheim (F-N) formula
we use here to predict the emitted current density is given in (\ref{eq:units})
\cite{BC} \cite{FN}
%
\begin{equation}\label{eq:units}
    J(\mathbf{r},t) = \frac{A(\beta E)^2}{\varphi t(y)^2}
                      \exp{\left(\frac{-B v(y)\varphi^{3/2}}{\beta E}\right)}
                      \left[\hbox{A/$m^2$}\right]
\end{equation}
%
where $J(\mathbf{r},t)$ stands for emitted electric current density in position
$\mathbf{r}$ and time $t$. The Greek letters $\varphi$ and $\beta$ denote the
work function of the surface material and the local field enhancement factor
respectively. The parameter $E$ is the electric field in the normal direction
of surface. The parameters $A$ and $B$ are empirical constants. The functions
$v(y)$ and $t(y)$ representing the image charge effects \cite{BC} as a function
of the Fowler-Nordheim parameter $y$ with the following definition\cite{DE}
%
\begin{equation}\label{eq:imagecharge}
    y = \sqrt{\frac{e^3}{4\pi\varepsilon}}\frac{\sqrt{\beta E}}{\varphi} 
      = 3.795\times10^{-5}\frac{\sqrt{\beta E}}{\varphi} \text{.}
\end{equation}
%
In our model, we have chosen a simpler approximation originated by J. H. Han\cite{DE}
\begin{eqnarray*}
v(y) &=& a-by^2 \\
t(y) &\approx& 1 \text{.}
\end{eqnarray*}
These approximations are valid for a large range of $y$, corresponding to
typical applied electric field ranges in RF guns.

Users can customize dark current simulation by specifying the value of the work
function $\varphi$, local field enhancement factor $\beta$ and other parameters
present in (\ref{eq:units}) and (\ref{eq:imagecharge}) in the \opal input file.

The first secondary emission model implemented in \opal is based on a
phenomenological model developed by M. A. Furman and M. Pivi\cite{SE}. This
choice was based on the self-consistency property this particular secondary
model offers. In this context self-consistency means that if we define one incident
electron and the followed secondary emission procedure as an event, the event
generator is constructed so that
%
\begin{enumerate}
    \item when averaging over an infinite number of secondary-emission events, 
    the reconstructed secondary emission yield $\delta$ and its energy spectrum
    $ d\delta/dE$ are guaranteed to agree with the corresponding input quantities 
    \item the energy integral of $d\delta/dE$ is guaranteed to equal $\delta$
    \item the energy of any given emitted electron is guaranteed not to exceed the 
    primary energy
    \item the aggregated energy of the electrons emitted in any multi-electron event 
    is also guaranteed not to exceed the primary energy.
\end{enumerate}


\begin{figure}
  \begin{center}
\includegraphics[width=0.4\textwidth]{HB2010Figure4.jpg}
\end{center}
    
    \caption{Basic computational procedure of secondary emission model.\label{fig:S-E}}
\end{figure}

The basic computational procedure of the Furman-Pivi's secondary emission model is shown in
Figure \ref{fig:S-E}. This model calculates the number of secondary electrons
that result from an incident electron of a given energy on a material at a
given angle (see Figure~\ref{incident electrons}). For each of the generated 
secondary electrons the associated process: {\em true secondary}, {\em rediffused} or
{\em backscattered} is recorded. 

\begin{figure}[H]
    \centering
    \input{figs/Incident.tikz}
    % \includegraphics[width=3 in]{incident_diagram.pdf}
    \caption{Geometry used by Furman-Pivi's secondary electrons emission model.}
    \label{incident electrons}
\end{figure}

The other secondary emission model we use is based on a secondary emission yield formula developed by Vaughan \cite{Vaughan, VaughanRv, FS}:
\begin{subequations}
\label{allequations}
\begin{eqnarray}
\delta(E,\theta)&=&\delta_0,\ \text{for}\ v \le 0 \label{eq:VaughanA} 
\\
    \delta(E,\theta)&=&\delta_{max}(\theta)\cdot (v e^{1-v})^k,\ \text{for}\ v \le 3.6 \label{eq:VaughanB} 
\\
\delta(E,\theta)&=&\delta_{max}(\theta)\cdot 1.125/v^{0.35},\ \text{for}\ v > 3.6 \label{eq:VaughanC} 
\end{eqnarray}
\end{subequations}
where 
\begin{eqnarray*}
v=\frac{\displaystyle E-E_0}{\displaystyle E_{max}(\theta)-E_0},
\end{eqnarray*}
\begin{eqnarray*}
k=0.56,\ \ \text{for}\ v<1,
\end{eqnarray*}
\begin{eqnarray*}
k=0.25,\ \ \text{for}\ 1<v\le{3.6},
\end{eqnarray*}
\begin{eqnarray*}
\delta_{max}(\theta)=\delta_{max}(0)\cdot (1+k_{\theta}\theta^2/2\pi),
\end{eqnarray*}
\begin{eqnarray*}
E_{max}(\theta)=E_{max}(0)\cdot (1+k_E\theta^2/2\pi).
\end{eqnarray*}
The secondary emission yield value for an impacting electron energy $E$ and incident angle $\theta$ w.r.t the surface normal is denoted as $\delta(E,\theta)$. Parameter $k_{\theta}$ and $k_E$ denotes the dependence on surface roughness. Both
should be assigned a default value of 1.0, which appears appropriate for typical dull surfaces in a working tube environment, and lower values down to zero or higher values, up to about 2.0, are only valid for specified cases \cite{Vaughan}. $E_{max}(0)$ is the impacting energy when incident angle is zero and secondary yield reaches its maximum value. $E_0$ is an adjustable parameter to make the first crossover energy at which the secondary yield equals to 1 be fitted to the experiment data \cite{FS}.

Motivated by the fact that the population of particles in simulation domain may continually grow exponentially and lead to tens of magnitude larger within limited simulation time steps, which may cause the exhaust of computing memory, a re-normal\\-ization of simulation particle number approach which maintains a constant number of simulation particles is also implemented. In each electron impacting events, instead of emitting the real number of simulation particles predicted by secondary emission models, this re-normalization approach emit only one particle, and the current of newly emitted particle will be the current of incident particle multiplied by SEY value $\delta$.    

Both the Furman-Pivi's model and Vaughan's model have been carefully benchmarked in both re-normalize simulation particle approach and real simulation particles approach against a non-stationary multipacting theory \cite{nonstationary}. The \opal simulation results and the theory match very well (see figure \ref{fig:PPFurman-Pivi} and figure \ref{fig:PPVaughan}).
\begin{figure}[ht]
 \begin{center}
 \includegraphics[width=1.1\linewidth,angle=0]{figs/const_particle_benchmark_FurmanPivi.pdf}
  \caption{Time evolution of electron number predicted by theoretical model and \opal\ simulation using Furman-Pivi's secondary emission model with both constant simulation particle approach and real emission particle approach at $f=200MHz$, $V_0=120V$, $d=5mm$}
  \label{fig:PPFurman-Pivi}
 \end{center}
\end{figure}  
\begin{figure}[ht]
 \begin{center}
 \includegraphics[width=1.1\linewidth,angle=0]{figs/const_particle_benchmark.pdf}
  \caption{Time evolution of electron number predicted by theoretical model and \opal\ simulation using Vaughan's secondary emission model with both constant simulation particle approach and real emission particle approach at $f=1640$MHz, $V_0=120$V, $d=1$mm.}
  \label{fig:PPVaughan}
 \end{center}
\end{figure}  

Currently we have used the feasible tool provided by \opal\ for studying the multipacting phenomena observed in the RF conditioning process of CYCIAE-100 MeV cyclotron \cite{ciae-rf-2013}. And very good agreements between the observed and \opal\ simulated multipacting zones have been achieved.


 




==> contrib/oblaapp.tex <==
% !TEX root = ../main.tex

% ckeck with Thomas
\begin{figure}[h!]
  \begin{center}
  \includegraphics[width=.95\columnwidth]{test}
    \end{center}
  \caption{test test.}
  \label{fig:name}
\end{figure}
\clearpage

==> contrib/ppbench.tex <==
% !TEX root = ../main.tex


==> contrib/qa.tex <==
% !TEX root = ../main.tex

\subsection{Quality Assurance (AG)}  \label{ssec:qa}


==> contrib/spiralapp.tex <==
% !TEX root = ../main.tex

